Light in the Larynx: a Miniaturized Robotic Optical Fiber for In-office Laser Surgery of the Vocal Folds

This letter reports the design, construction, and experimental validation of a novel hand-held robot for in-office laser surgery of the vocal folds. In-office endoscopic laser surgery is an emerging trend in Laryngology: It promises to deliver the same patient outcomes of traditional surgical treatment (i.e., in the operating room), at a fraction of the cost. Unfortunately, office procedures can be challenging to perform; the optical fibers used for laser delivery can only emit light forward in a line-of-sight fashion, which severely limits anatomical access. The robot we present in this letter aims to overcome these challenges. The end effector of the robot is a steerable laser fiber, created through the combination of a thin optical fiber (0.225 mm) with a tendon-actuated Nickel-Titanium notched sheath that provides bending. This device can be seamlessly used with most commercially available endoscopes, as it is sufficiently small (1.1 mm) to pass through a working channel. To control the fiber, we propose a compact actuation unit that can be mounted on top of the endoscope handle, so that, during a procedure, the operating physician can operate both the endoscope and the steerable fiber with a single hand. We report simulation and phantom experiments demonstrating that the proposed device substantially enhances surgical access compared to current clinical fibers.

==> coupling-system.tex <==
\subsection{Laser Coupling Module}
\AJC{add laser coupling section}
A 532 nm laser with a power up to 10W from the Aura-i Laser System (Laserscope® KTP/532, Boston Scientific Co.) was guided by an Endostat Surgical Fiber (10-0632, American Medical Systems). The glass core diameter of this multimode Endostat fiber is 0.4 mm and the minimum bending radius was measured to be 12mm. The large core diameter of the Endostat fiber and the resulting stiffness make the fiber difficult to bend, susceptible to light leaking when bent, and easy to break from sharp bending, all of which limit the steerability of the fiber. This challenge was solved by a home-made optical coupling system which couples the high-power laser from the Endostat fiber to a step-index multimode fiber (FP200ERT, Thorlabs) with a 0.2 mm glass core diameter, 0.225 mm glass cladding, and 0.5 mm polymer coating. With around a half of the core diameter of the Endostat fiber, this thinner multimode fiber can be readily bent with a 6 mm bending radius with only 4.5\% optical power loss and thus increases the flexibility of the probe system. The coupling system consists of two key components, a reflective collimator (RC08FC-P01, Thorlabs) and an achromatic straight collimator (F950FC-A, Thorlabs). The laser emitted from the Endostat fiber was collimated by the reflective collimator, propagated in free space, and then focused and coupled to the step-index multimode fiber by the straight collimator. We have achieved up to 54.5\% of the laser coupling effeciency between the two types of fiber and the performance of the system is consistent with limited effort of regular maintenance such as realignments. The detailed characterization of the coupling system can be found in []. The developed coupling system enables the light to be delivered by the thin multimode fiber and in turn the mechanical steering and control of the steerable probe.
